Nonlinear Schr\"odinger problems: symmetries of some variational solutions

In this paper, we are interested in the nonlinear Schr\"odinger problem $-\Delta u + Vu = \abs{u}^{p-2}u$ submitted to the Dirichlet boundary conditions. We consider $p>2$ and we are working with an open bounded domain $\Omega\subset\IR^N$ ($N\geq 2$). Potential $V$ satisfies $\max(V,0)\in L^{N/2}(\Omega)$ and $\min(V,0)\in L^{+\infty}(\Omega)$. Moreover, $-\Delta + V$ is positive definite and has one and only one principal eigenvalue. When $p\simeq 2$, we prove the uniqueness of the solution once we fix the projection on an eigenspace of $-\Delta + V$. It implies partial symmetries (or symmetry breaking) for ground state and least energy nodal solutions. In the litterature, the case $V\equiv 0$ has already been studied. Here, we generalize the technique at our case by pointing out and explaining differences. To finish, as illustration, we implement the (modified) mountain pass algorithm to work with $V$ negative, piecewise constant or not bounded. It permits us to exhibit direct examples where the solutions break down the symmetries of $V$.

==> rectV2posMPA.tex <==
\meshline{black}{0.5604}{-0.01067}{0.5601}{0.00762}
\meshline{black}{0.55818}{-0.04398}{0.5604}{-0.01067}
\meshline{black}{0.5569}{-0.05913}{0.55223}{-0.09525}
\meshline{black}{0.55223}{-0.09525}{0.54348}{-0.13479}
\meshline{black}{0.55963}{0.03262}{0.55637}{0.06667}
\meshline{black}{0.55963}{0.03262}{0.5601}{0.00762}\meshline{black}{0.55772}{-0.05325}{0.55818}{-0.04398}
\meshline{black}{0.5569}{-0.05913}{0.55772}{-0.05325}
\meshline{black}{0.53137}{-0.17729}{0.5425}{-0.13854}
\meshline{black}{0.54348}{-0.13479}{0.54312}{-0.13652}\meshline{black}{0.55528}{0.07661}{0.55637}{0.06667}\meshline{black}{0.54751}{0.11997}{0.55528}{0.07661}
\meshline{black}{0.54312}{-0.13652}{0.5425}{-0.13854}
\meshline{black}{0.53519}{0.16683}{0.54225}{0.13998}
\meshline{black}{0.53137}{-0.17729}{0.52153}{-0.20295}
\meshline{black}{0.53519}{0.16683}{0.5346}{0.16873}
\meshline{black}{0.54723}{0.12132}{0.54751}{0.11997}
\meshline{black}{0.54225}{0.13998}{0.54723}{0.12132}\meshline{black}{0.52153}{-0.20295}{0.516}{-0.21745}
\meshline{black}{0.51848}{0.21331}{0.5346}{0.16873}
\meshline{black}{0.51848}{0.21331}{0.51831}{0.21372}
\meshline{black}{0.50091}{-0.24896}{0.4973}{-0.25683}
\meshline{black}{0.516}{-0.21745}{0.50091}{-0.24896}
\meshline{black}{0.4973}{-0.25683}{0.4956}{-0.2599}
\meshline{black}{0.51831}{0.21372}{0.51697}{0.21658}
\meshline{black}{0.49917}{0.25551}{0.51697}{0.21658}
\meshline{black}{0.4956}{-0.2599}{0.47538}{-0.29542}
\meshline{black}{0.46678}{-0.30841}{0.47538}{-0.29542}
\meshline{black}{0.49628}{0.26091}{0.49917}{0.25551}\meshline{black}{0.49628}{0.26091}{0.47747}{0.2944}
\meshline{black}{0.46678}{-0.30841}{0.4495}{-0.33321}
\meshline{black}{0.47747}{0.2944}{0.46724}{0.30988}
\meshline{black}{0.46724}{0.30988}{0.45338}{0.3305}
\meshline{black}{0.4495}{-0.33321}{0.43579}{-0.35066}
\meshline{black}{0.45338}{0.3305}{0.42949}{0.36056}
\meshline{black}{0.43579}{-0.35066}{0.41913}{-0.37035}
\meshline{black}{0.4269}{0.36383}{0.42949}{0.36056}
\meshline{black}{0.40276}{-0.38797}{0.41913}{-0.37035}
\meshline{black}{0.42255}{0.36847}{0.4269}{0.36383}
\meshline{black}{0.40276}{-0.38797}{0.38393}{-0.4064}\meshline{black}{0.39856}{0.395}{0.42255}{0.36847}
\meshline{black}{0.36828}{-0.42068}{0.38393}{-0.4064}
\meshline{black}{0.37794}{0.41409}{0.39856}{0.395}\meshline{black}{0.37794}{0.41409}{0.36793}{0.42361}
\meshline{black}{0.36828}{-0.42068}{0.34332}{-0.44094}
\meshline{black}{0.36793}{0.42361}{0.35753}{0.43189}
\meshline{black}{0.33299}{-0.44898}{0.34332}{-0.44094}
\meshline{black}{0.33529}{0.45004}{0.35753}{0.43189}\meshline{black}{0.33299}{-0.44898}{0.29865}{-0.47177}
\meshline{black}{0.29865}{-0.47177}{0.29239}{-0.47605}
\meshline{black}{0.33529}{0.45004}{0.30155}{0.47294}
\meshline{black}{0.30155}{0.47294}{0.30021}{0.47389}
\meshline{black}{0.29239}{-0.47605}{0.29074}{-0.47703}
\meshline{black}{0.30021}{0.47389}{0.29936}{0.47439}
\meshline{black}{0.28159}{-0.48193}{0.29074}{-0.47703}
\meshline{black}{0.24786}{-0.50047}{0.28159}{-0.48193}
\meshline{black}{0.29936}{0.47439}{0.2632}{0.49568}
\meshline{black}{0.2632}{0.49568}{0.24513}{0.5045}
\meshline{black}{0.2398}{-0.50417}{0.24786}{-0.50047}
\meshline{black}{0.20739}{-0.51836}{0.2398}{-0.50417}
\meshline{black}{0.22361}{0.51475}{0.24513}{0.5045}\meshline{black}{0.1918}{-0.52409}{0.20739}{-0.51836}
\meshline{black}{0.1934}{0.5266}{0.22361}{0.51475}
\meshline{black}{0.1918}{-0.52409}{0.16552}{-0.53298}
\meshline{black}{0.18143}{0.531}{0.1934}{0.5266}
\meshline{black}{0.16552}{-0.53298}{0.14388}{-0.53897}
\meshline{black}{0.14363}{0.54236}{0.18143}{0.531}
\meshline{black}{0.11867}{-0.54498}{0.14388}{-0.53897}
\meshline{black}{0.13648}{0.54424}{0.14363}{0.54236}\meshline{black}{0.09267}{-0.55003}{0.11867}{-0.54498}
\meshline{black}{0.13648}{0.54424}{0.09545}{0.55291}
\meshline{black}{0.06374}{-0.5537}{0.09267}{-0.55003}
\meshline{black}{0.08843}{0.55405}{0.09545}{0.55291}
\meshline{black}{0.05322}{-0.55484}{0.06374}{-0.5537}
\meshline{black}{0.04865}{0.55905}{0.08843}{0.55405}
\meshline{black}{0.05322}{-0.55484}{0.02212}{-0.55696}
\meshline{black}{0.03679}{0.55983}{0.04865}{0.55905}\meshline{black}{0.00212}{-0.55706}{0.02212}{-0.55696}
\meshline{black}{-0.02354}{-0.55675}{0.00212}{-0.55706}
\meshline{black}{0.03679}{0.55983}{0.00314}{0.56125}
\meshline{black}{-0.02354}{-0.55675}{-0.05247}{-0.55451}
\meshline{black}{0.00314}{0.56125}{-0.01919}{0.56064}
\meshline{black}{-0.06943}{-0.55274}{-0.05247}{-0.55451}
\meshline{black}{-0.01919}{0.56064}{-0.04109}{0.55979}
\meshline{black}{-0.1028}{-0.54744}{-0.06943}{-0.55274}
\meshline{black}{-0.11618}{-0.54477}{-0.1028}{-0.54744}
\meshline{black}{-0.04109}{0.55979}{-0.08067}{0.55517}
\meshline{black}{-0.14934}{-0.53673}{-0.11618}{-0.54477}
\meshline{black}{-0.14934}{-0.53673}{-0.16437}{-0.53226}
\meshline{black}{-0.08067}{0.55517}{-0.08404}{0.55478}
\meshline{black}{-0.16437}{-0.53226}{-0.19282}{-0.52291}
\meshline{black}{-0.19282}{-0.52291}{-0.21463}{-0.51418}
\meshline{black}{-0.12605}{0.54695}{-0.08969}{0.55364}\meshline{black}{-0.08404}{0.55478}{-0.08969}{0.55364}
\meshline{black}{-0.12605}{0.54695}{-0.15052}{0.54018}
\meshline{black}{-0.21463}{-0.51418}{-0.23367}{-0.50623}
\meshline{black}{-0.26772}{-0.48898}{-0.23367}{-0.50623}
\meshline{black}{-0.28002}{-0.48185}{-0.30854}{-0.46494}\meshline{black}{-0.15052}{0.54018}{-0.16694}{0.53584}
\meshline{black}{-0.27208}{-0.48675}{-0.26772}{-0.48898}
\meshline{black}{-0.30854}{-0.46494}{-0.32475}{-0.45332}\meshline{black}{-0.28002}{-0.48185}{-0.27208}{-0.48675}
\meshline{black}{-0.20679}{0.52176}{-0.1839}{0.52969}
\meshline{black}{-0.16694}{0.53584}{-0.1839}{0.52969}
\meshline{black}{-0.34285}{-0.44059}{-0.32475}{-0.45332}
\meshline{black}{-0.36276}{-0.42377}{-0.37505}{-0.4137}\meshline{black}{-0.23376}{0.50961}{-0.20679}{0.52176}
\meshline{black}{-0.36276}{-0.42377}{-0.34285}{-0.44059}
\meshline{black}{-0.37505}{-0.4137}{-0.38724}{-0.40173}
\meshline{black}{-0.23376}{0.50961}{-0.24551}{0.50456}
\meshline{black}{-0.38724}{-0.40173}{-0.40532}{-0.38452}
\meshline{black}{-0.25314}{0.50047}{-0.28318}{0.48455}
\meshline{black}{-0.43345}{-0.35283}{-0.41784}{-0.37031}
\meshline{black}{-0.24551}{0.50456}{-0.25314}{0.50047}
\meshline{black}{-0.41784}{-0.37031}{-0.40532}{-0.38452}
\meshline{black}{-0.45872}{-0.31917}{-0.45926}{-0.31845}\meshline{black}{-0.45872}{-0.31917}{-0.43345}{-0.35283}
\meshline{black}{-0.3196}{0.46117}{-0.30834}{0.46846}\meshline{black}{-0.28318}{0.48455}{-0.30834}{0.46846}
\meshline{black}{-0.45926}{-0.31845}{-0.46062}{-0.31629}\meshline{black}{-0.35484}{0.4344}{-0.35434}{0.43479}
\meshline{black}{-0.35434}{0.43479}{-0.3196}{0.46117}
\meshline{black}{-0.46062}{-0.31629}{-0.48304}{-0.28177}
\meshline{black}{-0.35798}{0.43157}{-0.35484}{0.4344}
\meshline{black}{-0.48968}{-0.26975}{-0.50424}{-0.24222}\meshline{black}{-0.48304}{-0.28177}{-0.48968}{-0.26975}
\meshline{black}{-0.38899}{0.40413}{-0.35798}{0.43157}
\meshline{black}{-0.5135}{-0.22175}{-0.52269}{-0.19965}\meshline{black}{-0.50424}{-0.24222}{-0.5135}{-0.22175}
\meshline{black}{-0.42188}{0.36956}{-0.39329}{0.39989}
\meshline{black}{-0.38899}{0.40413}{-0.39329}{0.39989}
\meshline{black}{-0.5315}{-0.17504}{-0.53812}{-0.15367}\meshline{black}{-0.52269}{-0.19965}{-0.5315}{-0.17504}
\meshline{black}{-0.4829}{0.28479}{-0.48051}{0.289}\meshline{black}{-0.48051}{0.289}{-0.46691}{0.30954}
\meshline{black}{-0.42678}{0.3639}{-0.45331}{0.33007}
\meshline{black}{-0.42188}{0.36956}{-0.42678}{0.3639}
\meshline{black}{-0.54464}{-0.12941}{-0.55007}{-0.10352}
\meshline{black}{-0.53812}{-0.15367}{-0.54464}{-0.12941}
\meshline{black}{-0.4829}{0.28479}{-0.50186}{0.25029}
\meshline{black}{-0.50186}{0.25029}{-0.51004}{0.23223}
\meshline{black}{-0.45564}{0.32691}{-0.46691}{0.30954}
\meshline{black}{-0.45331}{0.33007}{-0.45564}{0.32691}
\meshline{black}{-0.53387}{0.17052}{-0.53374}{0.17089}
\meshline{black}{-0.53387}{0.17052}{-0.53394}{0.17028}
\meshline{black}{-0.55976}{0.01361}{-0.56017}{0.00314}
\meshline{black}{-0.55914}{-0.02076}{-0.56017}{0.00314}\meshline{black}{-0.55778}{-0.04822}{-0.55356}{-0.08459}
\meshline{black}{-0.55356}{-0.08459}{-0.55007}{-0.10352}
\meshline{black}{-0.51004}{0.23223}{-0.51967}{0.2108}
\meshline{black}{-0.51967}{0.2108}{-0.53374}{0.17089}
\meshline{black}{-0.53394}{0.17028}{-0.54544}{0.1297}
\meshline{black}{-0.54544}{0.1297}{-0.55246}{0.0925}
\meshline{black}{-0.55856}{0.04602}{-0.55379}{0.08429}\meshline{black}{-0.55856}{0.04602}{-0.55976}{0.01361}
\meshline{black}{-0.55914}{-0.02076}{-0.55859}{-0.04041}
\meshline{black}{-0.55859}{-0.04041}{-0.55778}{-0.04822}
\meshline{black}{-0.55246}{0.0925}{-0.55335}{0.08815}
\meshline{black}{-0.55335}{0.08815}{-0.55379}{0.08429}
\meshline{black}{0.74614}{-0.03709}{0.74566}{-0.05013}
\meshline{black}{0.74329}{-0.07268}{0.74566}{-0.05013}
\meshline{black}{0.74666}{0.02731}{0.74749}{-0.00642}
\meshline{black}{0.74749}{-0.00642}{0.74614}{-0.03709}
\meshline{black}{0.74284}{0.08193}{0.74382}{0.06808}
\meshline{black}{0.74284}{0.08193}{0.74225}{0.0865}
\meshline{black}{0.74329}{-0.07268}{0.74165}{-0.09196}\meshline{black}{0.73534}{-0.13382}{0.73958}{-0.1046}
\meshline{black}{0.74644}{0.03789}{0.74666}{0.02731}\meshline{black}{0.74644}{0.03789}{0.74382}{0.06808}
\meshline{black}{0.74165}{-0.09196}{0.73958}{-0.1046}\meshline{black}{0.72706}{-0.17087}{0.73534}{-0.13382}
\meshline{black}{0.73682}{0.12605}{0.74225}{0.0865}
\meshline{black}{0.73682}{0.12605}{0.73415}{0.14008}
\meshline{black}{0.7263}{-0.17467}{0.72706}{-0.17087}
\meshline{black}{0.72772}{0.17108}{0.73415}{0.14008}
\meshline{black}{0.72282}{0.19043}{0.72772}{0.17108}
\meshline{black}{0.71692}{-0.21044}{0.72542}{-0.17781}
\meshline{black}{0.72542}{-0.17781}{0.7263}{-0.17467}
\meshline{black}{0.7091}{-0.23435}{0.71692}{-0.21044}
\meshline{black}{0.71531}{0.21723}{0.72282}{0.19043}\meshline{black}{0.70857}{0.2383}{0.71531}{0.21723}
\meshline{black}{0.7091}{-0.23435}{0.70576}{-0.24474}
\meshline{black}{0.6936}{-0.27703}{0.69682}{-0.26814}
\meshline{black}{0.69682}{-0.26814}{0.70576}{-0.24474}
\meshline{black}{0.69937}{0.26405}{0.70857}{0.2383}\meshline{black}{0.6936}{-0.27703}{0.69127}{-0.28234}
\meshline{black}{0.69178}{0.28354}{0.69937}{0.26405}
\meshline{black}{0.68}{-0.30958}{0.69127}{-0.28234}
\meshline{black}{0.67943}{0.31174}{0.69178}{0.28354}
\meshline{black}{0.68}{-0.30958}{0.66187}{-0.34503}
\meshline{black}{0.67943}{0.31174}{0.67261}{0.32647}
\meshline{black}{0.66187}{-0.34503}{0.65689}{-0.35535}
\meshline{black}{0.65411}{-0.36025}{0.65689}{-0.35535}
\meshline{black}{0.65498}{0.36019}{0.67261}{0.32647}
\meshline{black}{0.65138}{0.36685}{0.65498}{0.36019}
\meshline{black}{0.62884}{-0.40267}{0.65411}{-0.36025}
\meshline{black}{0.65138}{0.36685}{0.63781}{0.38903}
\meshline{black}{0.62884}{-0.40267}{0.62794}{-0.40407}
\meshline{black}{0.63781}{0.38903}{0.62856}{0.4047}
\meshline{black}{0.62794}{-0.40407}{0.60161}{-0.44204}\meshline{black}{0.62556}{0.40912}{0.62856}{0.4047}
\meshline{black}{0.60104}{-0.44282}{0.60161}{-0.44204}
\meshline{black}{0.60444}{0.44033}{0.62556}{0.40912}
\meshline{black}{0.5892}{-0.45773}{0.60104}{-0.44282}
\meshline{black}{0.60444}{0.44033}{0.59008}{0.4588}
\meshline{black}{0.57198}{-0.47957}{0.5892}{-0.45773}
\meshline{black}{0.59008}{0.4588}{0.57891}{0.47337}
\meshline{black}{0.5711}{-0.4806}{0.57198}{-0.47957}
\meshline{black}{0.55922}{0.4957}{0.57891}{0.47337}
\meshline{black}{0.54182}{-0.51337}{0.5711}{-0.4806}
\meshline{black}{0.55186}{0.50442}{0.55922}{0.4957}
\meshline{black}{0.53953}{-0.51572}{0.54182}{-0.51337}
\meshline{black}{0.54637}{0.51002}{0.55186}{0.50442}
\meshline{black}{0.54637}{0.51002}{0.52343}{0.53423}
\meshline{black}{0.51078}{-0.54408}{0.53953}{-0.51572}
\meshline{black}{0.51078}{-0.54408}{0.50921}{-0.54557}\meshline{black}{0.52343}{0.53423}{0.49512}{0.55996}
\meshline{black}{0.49512}{0.55996}{0.49276}{0.56219}
\meshline{black}{0.50921}{-0.54557}{0.47727}{-0.5734}
\meshline{black}{0.47727}{-0.5734}{0.47547}{-0.57498}
\meshline{black}{0.49011}{0.56434}{0.49276}{0.56219}
\meshline{black}{0.47547}{-0.57498}{0.47537}{-0.57507}
\meshline{black}{0.46079}{0.58914}{0.49011}{0.56434}
\meshline{black}{0.43654}{-0.6049}{0.45143}{-0.59345}
\meshline{black}{0.47537}{-0.57507}{0.45143}{-0.59345}
\meshline{black}{0.43647}{-0.60495}{0.43654}{-0.6049}
\meshline{black}{0.43525}{0.60765}{0.46079}{0.58914}
\meshline{black}{0.42662}{0.61411}{0.43525}{0.60765}
\meshline{black}{0.39805}{-0.63091}{0.43647}{-0.60495}
\meshline{black}{0.41198}{0.62344}{0.42662}{0.61411}
\meshline{black}{0.3932}{-0.6338}{0.39805}{-0.63091}
\meshline{black}{0.41198}{0.62344}{0.39084}{0.63757}
\meshline{black}{0.36217}{-0.65202}{0.3932}{-0.6338}
\meshline{black}{0.39084}{0.63757}{0.37827}{0.64475}
\meshline{black}{0.37827}{0.64475}{0.35331}{0.65923}
\meshline{black}{0.36217}{-0.65202}{0.35407}{-0.65644}
\meshline{black}{0.32388}{0.6738}{0.35331}{0.65923}
\meshline{black}{0.35407}{-0.65644}{0.32112}{-0.67292}
\meshline{black}{0.31388}{0.67874}{0.32388}{0.6738}
\meshline{black}{0.32112}{-0.67292}{0.31348}{-0.67654}\meshline{black}{0.27534}{0.69496}{0.31388}{0.67874}\meshline{black}{0.27493}{-0.6928}{0.31348}{-0.67654}
\meshline{black}{0.27534}{0.69496}{0.27267}{0.69613}
\meshline{black}{0.26982}{-0.69481}{0.27493}{-0.6928}
\meshline{black}{0.27267}{0.69613}{0.27196}{0.6964}
\meshline{black}{0.22682}{-0.70969}{0.26982}{-0.69481}
\meshline{black}{0.22968}{0.71162}{0.27196}{0.6964}\meshline{black}{0.22407}{-0.71055}{0.22682}{-0.70969}
\meshline{black}{0.22968}{0.71162}{0.22216}{0.71396}
\meshline{black}{0.17866}{-0.72295}{0.22407}{-0.71055}
\meshline{black}{0.18398}{0.72481}{0.22216}{0.71396}\meshline{black}{0.17673}{-0.72341}{0.17866}{-0.72295}
\meshline{black}{0.18398}{0.72481}{0.17336}{0.72741}
\meshline{black}{0.13497}{0.73549}{0.17336}{0.72741}
\meshline{black}{0.13117}{-0.73266}{0.17673}{-0.72341}
\meshline{black}{0.12779}{-0.73321}{0.13117}{-0.73266}
\meshline{black}{0.12404}{0.73744}{0.13497}{0.73549}
\meshline{black}{0.08304}{0.74312}{0.12404}{0.73744}
\meshline{black}{0.08441}{-0.73905}{0.12779}{-0.73321}
\meshline{black}{0.08441}{-0.73905}{0.0782}{-0.73962}\meshline{black}{0.07445}{0.7441}{0.08304}{0.74312}
\meshline{black}{0.02709}{0.74715}{0.07445}{0.7441}\meshline{black}{0.03938}{-0.74232}{0.0782}{-0.73962}
\meshline{black}{0.03938}{-0.74232}{0.0315}{-0.74256}
\meshline{black}{0.02709}{0.74715}{0.02502}{0.74725}
\meshline{black}{-0.02512}{0.74723}{0.01089}{0.74715}
\meshline{black}{0.0315}{-0.74256}{-0.0038}{-0.74271}
\meshline{black}{0.02502}{0.74725}{0.01089}{0.74715}
\meshline{black}{-0.0038}{-0.74271}{-0.00978}{-0.74268}\meshline{black}{-0.02974}{0.74701}{-0.02512}{0.74723}
\meshline{black}{-0.05037}{-0.74038}{-0.00978}{-0.74268}
\meshline{black}{-0.02974}{0.74701}{-0.06812}{0.74463}
\meshline{black}{-0.05301}{-0.74025}{-0.05037}{-0.74038}
\meshline{black}{-0.07538}{0.7438}{-0.06812}{0.74463}
\meshline{black}{-0.05346}{-0.74021}{-0.05301}{-0.74025}
\meshline{black}{-0.05346}{-0.74021}{-0.09775}{-0.73548}\meshline{black}{-0.07538}{0.7438}{-0.10319}{0.74083}
\meshline{black}{-0.14373}{0.73366}{-0.10319}{0.74083}\meshline{black}{-0.09775}{-0.73548}{-0.10403}{-0.73455}
\meshline{black}{-0.10403}{-0.73455}{-0.14358}{-0.72787}\meshline{black}{-0.14373}{0.73366}{-0.14425}{0.73357}
\meshline{black}{-0.15219}{-0.72614}{-0.14358}{-0.72787}
\meshline{black}{-0.15219}{-0.72614}{-0.19048}{-0.71721}\meshline{black}{-0.18541}{0.72465}{-0.14483}{0.73343}
\meshline{black}{-0.14483}{0.73343}{-0.14425}{0.73357}
\meshline{black}{-0.19784}{-0.71533}{-0.19048}{-0.71721}
\meshline{black}{-0.19784}{-0.71533}{-0.23887}{-0.70302}
\meshline{black}{-0.22166}{0.71391}{-0.18541}{0.72465}
\meshline{black}{-0.25258}{-0.69808}{-0.2829}{-0.68724}\meshline{black}{-0.28928}{-0.68453}{-0.2829}{-0.68724}
\meshline{black}{-0.24129}{-0.70227}{-0.23887}{-0.70302}
\meshline{black}{-0.25258}{-0.69808}{-0.24129}{-0.70227}
\meshline{black}{-0.22166}{0.71391}{-0.2257}{0.7128}
\meshline{black}{-0.32274}{-0.67027}{-0.28928}{-0.68453}
\meshline{black}{-0.34237}{-0.66033}{-0.32274}{-0.67027}
\meshline{black}{-0.26582}{0.69916}{-0.22926}{0.71152}\meshline{black}{-0.2257}{0.7128}{-0.22926}{0.71152}
\meshline{black}{-0.39728}{-0.62968}{-0.39377}{-0.63165}
\meshline{black}{-0.39728}{-0.62968}{-0.39926}{-0.62836}\meshline{black}{-0.30077}{0.68432}{-0.30562}{0.68236}
\meshline{black}{-0.36078}{-0.65116}{-0.34237}{-0.66033}
\meshline{black}{-0.26582}{0.69916}{-0.30077}{0.68432}
\meshline{black}{-0.39377}{-0.63165}{-0.36078}{-0.65116}
\meshline{black}{-0.39926}{-0.62836}{-0.43286}{-0.60666}
\meshline{black}{-0.31295}{0.6787}{-0.30562}{0.68236}
\meshline{black}{-0.45953}{-0.58637}{-0.43286}{-0.60666}
\meshline{black}{-0.49847}{-0.55473}{-0.4739}{-0.57491}
\meshline{black}{-0.34513}{0.6635}{-0.31295}{0.6787}
\meshline{black}{-0.46646}{-0.5813}{-0.45953}{-0.58637}
\meshline{black}{-0.49847}{-0.55473}{-0.52326}{-0.53087}\meshline{black}{-0.46646}{-0.5813}{-0.4739}{-0.57491}
\meshline{black}{-0.38384}{0.64187}{-0.36318}{0.65328}
\meshline{black}{-0.34513}{0.6635}{-0.36318}{0.65328}
\meshline{black}{-0.53303}{-0.52125}{-0.55827}{-0.49509}
\meshline{black}{-0.52888}{-0.5257}{-0.52326}{-0.53087}
\meshline{black}{-0.58042}{-0.46842}{-0.58542}{-0.46254}\meshline{black}{-0.52888}{-0.5257}{-0.53303}{-0.52125}
\meshline{black}{-0.55827}{-0.49509}{-0.58042}{-0.46842}
\meshline{black}{-0.42017}{0.61833}{-0.41816}{0.61961}\meshline{black}{-0.41816}{0.61961}{-0.38384}{0.64187}
\meshline{black}{-0.58542}{-0.46254}{-0.59465}{-0.44993}
\meshline{black}{-0.4256}{0.61432}{-0.42017}{0.61833}\meshline{black}{-0.61119}{-0.42829}{-0.59465}{-0.44993}
\meshline{black}{-0.61816}{-0.41781}{-0.6358}{-0.39128}
\meshline{black}{-0.4256}{0.61432}{-0.45504}{0.59335}
\meshline{black}{-0.61119}{-0.42829}{-0.61816}{-0.41781}
\meshline{black}{-0.65003}{-0.36663}{-0.65856}{-0.35169}
\meshline{black}{-0.65003}{-0.36663}{-0.6358}{-0.39128}
\meshline{black}{-0.48803}{0.56657}{-0.46427}{0.58591}\meshline{black}{-0.45504}{0.59335}{-0.46427}{0.58591}
\meshline{black}{-0.67674}{-0.31496}{-0.67872}{-0.31084}
\meshline{black}{-0.67674}{-0.31496}{-0.65856}{-0.35169}
\meshline{black}{-0.50264}{0.55348}{-0.52002}{0.53727}
\meshline{black}{-0.48803}{0.56657}{-0.50264}{0.55348}
\meshline{black}{-0.68891}{-0.28644}{-0.67872}{-0.31084}
\meshline{black}{-0.55337}{0.50276}{-0.53674}{0.52056}\meshline{black}{-0.53674}{0.52056}{-0.52002}{0.53727}
\meshline{black}{-0.69672}{-0.26823}{-0.68891}{-0.28644}
\meshline{black}{-0.58694}{0.46303}{-0.56932}{0.48473}
\meshline{black}{-0.55337}{0.50276}{-0.56932}{0.48473}
\meshline{black}{-0.71225}{-0.22425}{-0.698}{-0.26483}
\meshline{black}{-0.698}{-0.26483}{-0.69672}{-0.26823}
\meshline{black}{-0.5998}{0.44645}{-0.61849}{0.41987}
\meshline{black}{-0.5998}{0.44645}{-0.58694}{0.46303}
\meshline{black}{-0.73342}{-0.14068}{-0.7326}{-0.14553}
\meshline{black}{-0.73082}{-0.15296}{-0.7326}{-0.14553}
\meshline{black}{-0.72402}{-0.18377}{-0.7152}{-0.21442}
\meshline{black}{-0.7152}{-0.21442}{-0.71225}{-0.22425}
\meshline{black}{-0.67392}{0.32304}{-0.67076}{0.32999}
\meshline{black}{-0.67076}{0.32999}{-0.66004}{0.34989}
\meshline{black}{-0.62705}{0.40719}{-0.64712}{0.37404}
\meshline{black}{-0.61849}{0.41987}{-0.62705}{0.40719}
\meshline{black}{-0.73082}{-0.15296}{-0.72402}{-0.18377}
\meshline{black}{-0.74359}{-0.07037}{-0.74054}{-0.10059}
\meshline{black}{-0.74054}{-0.10059}{-0.73342}{-0.14068}
\meshline{black}{-0.68876}{0.29104}{-0.67392}{0.32304}
\meshline{black}{-0.69973}{0.2621}{-0.68876}{0.29104}
\meshline{black}{-0.65043}{0.36843}{-0.66004}{0.34989}
\meshline{black}{-0.65043}{0.36843}{-0.64712}{0.37404}
\meshline{black}{-0.71803}{0.20791}{-0.70996}{0.23217}
\meshline{black}{-0.71803}{0.20791}{-0.72245}{0.19009}
\meshline{black}{-0.73718}{0.12287}{-0.73489}{0.13396}\meshline{black}{-0.73718}{0.12287}{-0.73864}{0.11127}
\meshline{black}{-0.74468}{0.05853}{-0.74635}{0.03904}
\meshline{black}{-0.74686}{0.00028}{-0.74635}{0.03904}
\meshline{black}{-0.74553}{-0.05069}{-0.74696}{-0.00717}
\meshline{black}{-0.74553}{-0.05069}{-0.74359}{-0.07037}
\meshline{black}{-0.70443}{0.25021}{-0.69973}{0.2621}
\meshline{black}{-0.70443}{0.25021}{-0.70996}{0.23217}
\meshline{black}{-0.72919}{0.16479}{-0.72245}{0.19009}
\meshline{black}{-0.73489}{0.13396}{-0.72919}{0.16479}
\meshline{black}{-0.73864}{0.11127}{-0.74303}{0.08131}
\meshline{black}{-0.74303}{0.08131}{-0.74468}{0.05853}
\meshline{black}{-0.74686}{0.00028}{-0.74703}{-0.00482}
\meshline{black}{-0.74703}{-0.00482}{-0.74696}{-0.00717}
\meshline{black}{1}{0}{0.99529}{-0.04779}
\meshline{black}{1}{0}{0.9951}{0.04976}
\meshline{black}{0.99054}{-0.09606}{0.99529}{-0.04779}
\meshline{black}{0.9951}{0.04976}{0.99025}{0.09903}
\meshline{black}{0.98569}{-0.14533}{0.99054}{-0.09606}
\meshline{black}{0.99025}{0.09903}{0.98549}{0.1473}
\meshline{black}{0.98078}{-0.19509}{0.98569}{-0.14533}
\meshline{black}{0.98549}{0.1473}{0.98078}{0.19509}
\meshline{black}{0.96685}{-0.24104}{0.98078}{-0.19509}
\meshline{black}{0.98078}{0.19509}{0.96627}{0.24294}
\meshline{black}{0.95276}{-0.28746}{0.96685}{-0.24104}
\meshline{black}{0.96627}{0.24294}{0.9519}{0.29031}
\meshline{black}{0.93839}{-0.33483}{0.95276}{-0.28746}
\meshline{black}{0.9519}{0.29031}{0.93781}{0.33673}
\meshline{black}{0.92388}{-0.38268}{0.93839}{-0.33483}
\meshline{black}{0.93781}{0.33673}{0.92387}{0.38268}
\meshline{black}{0.90124}{-0.42503}{0.92388}{-0.38268}
\meshline{black}{0.92387}{0.38268}{0.9003}{0.42678}
\meshline{black}{0.87837}{-0.46781}{0.90124}{-0.42503}
\meshline{black}{0.9003}{0.42678}{0.87696}{0.47044}
\meshline{black}{0.85504}{-0.51147}{0.87837}{-0.46781}
\meshline{black}{0.87696}{0.47044}{0.8541}{0.51322}
\meshline{black}{0.83147}{-0.55557}{0.85504}{-0.51147}
\meshline{black}{0.8541}{0.51322}{0.83146}{0.55557}
\meshline{black}{0.80101}{-0.59269}{0.83147}{-0.55557}
\meshline{black}{0.83146}{0.55557}{0.79974}{0.59422}
\meshline{black}{0.77023}{-0.63018}{0.80101}{-0.59269}
\meshline{black}{0.79974}{0.59422}{0.76833}{0.63249}
\meshline{black}{0.73883}{-0.66845}{0.77023}{-0.63018}
\meshline{black}{0.76833}{0.63249}{0.73756}{0.66999}
\meshline{black}{0.70711}{-0.7071}{0.73883}{-0.66845}
\meshline{black}{0.73756}{0.66999}{0.7071}{0.7071}
\meshline{black}{0.66999}{-0.73756}{0.70711}{-0.7071}
\meshline{black}{0.7071}{0.7071}{0.66839}{0.73875}
\meshline{black}{0.63249}{-0.76834}{0.66999}{-0.73756}
\meshline{black}{0.66839}{0.73875}{0.6301}{0.77006}
\meshline{black}{0.59422}{-0.79974}{0.63249}{-0.76834}
\meshline{black}{0.6301}{0.77006}{0.59263}{0.8007}
\meshline{black}{0.55557}{-0.83146}{0.59422}{-0.79974}
\meshline{black}{0.59263}{0.8007}{0.55557}{0.831}
\meshline{black}{0.51323}{-0.85407}{0.55557}{-0.83146}
\meshline{black}{0.55557}{0.831}{0.51152}{0.85465}
\meshline{black}{0.47045}{-0.87692}{0.51323}{-0.85407}
\meshline{black}{0.51152}{0.85465}{0.46788}{0.87807}
\meshline{black}{0.42679}{-0.90024}{0.47045}{-0.87692}
\meshline{black}{0.46788}{0.87807}{0.42507}{0.90105}
\meshline{black}{0.38268}{-0.9238}{0.42679}{-0.90024}
\meshline{black}{0.42507}{0.90105}{0.38268}{0.9238}
\meshline{black}{0.33673}{-0.93776}{0.38268}{-0.9238}
\meshline{black}{0.38268}{0.9238}{0.33484}{0.93831}
\meshline{black}{0.2903}{-0.95186}{0.33673}{-0.93776}
\meshline{black}{0.33484}{0.93831}{0.28746}{0.95268}
\meshline{black}{0.24293}{-0.96625}{0.2903}{-0.95186}
\meshline{black}{0.28746}{0.95268}{0.24104}{0.96676}
\meshline{black}{0.19509}{-0.98078}{0.24293}{-0.96625}
\meshline{black}{0.24104}{0.96676}{0.19509}{0.9807}
\meshline{black}{0.1473}{-0.98549}{0.19509}{-0.98078}
\meshline{black}{0.19509}{0.9807}{0.14533}{0.98562}
\meshline{black}{0.09902}{-0.99024}{0.1473}{-0.98549}
\meshline{black}{0.14533}{0.98562}{0.09607}{0.9905}
\meshline{black}{0.04976}{-0.9951}{0.09902}{-0.99024}
\meshline{black}{0.09607}{0.9905}{0.04779}{0.99527}
\meshline{black}{0}{-1}{0.04976}{-0.9951}
\meshline{black}{0.04779}{0.99527}{0}{1}
\meshline{black}{-0.05951}{-0.98078}{0}{-1}
\meshline{black}{0}{1}{-0.04976}{0.9951}
\meshline{black}{-0.1026}{-0.97319}{-0.05951}{-0.98078}
\meshline{black}{-0.04976}{0.9951}{-0.09901}{0.99024}
\meshline{black}{-0.14672}{-0.96542}{-0.1026}{-0.97319}
\meshline{black}{-0.09901}{0.99024}{-0.14726}{0.98549}
\meshline{black}{-0.195}{0.98078}{-0.24283}{0.96622}
\meshline{black}{-0.14726}{0.98549}{-0.195}{0.98078}
\meshline{black}{-0.19186}{-0.95747}{-0.14672}{-0.96542}
\meshline{black}{-0.24283}{0.96622}{-0.29013}{0.95183}
\meshline{black}{-0.23803}{-0.94934}{-0.19186}{-0.95747}
\meshline{black}{-0.29013}{0.95183}{-0.33633}{0.93777}
\meshline{black}{-0.28522}{-0.94103}{-0.23803}{-0.94934}
\meshline{black}{-0.33633}{0.93777}{-0.382}{0.92387}
\meshline{black}{-0.33344}{-0.93254}{-0.28522}{-0.94103}
\meshline{black}{-0.382}{0.92387}{-0.4261}{0.90031}
\meshline{black}{-0.38268}{-0.92387}{-0.33344}{-0.93254}
\meshline{black}{-0.42503}{-0.90123}{-0.38268}{-0.92387}
\meshline{black}{-0.46781}{-0.87837}{-0.42503}{-0.90123}
\meshline{black}{-0.4261}{0.90031}{-0.46978}{0.87698}
\meshline{black}{-0.51147}{-0.85503}{-0.46781}{-0.87837}
\meshline{black}{-0.46978}{0.87698}{-0.5126}{0.85411}
\meshline{black}{-0.55557}{-0.83146}{-0.51147}{-0.85503}
\meshline{black}{-0.59268}{-0.801}{-0.55557}{-0.83146}
\meshline{black}{-0.63018}{-0.77023}{-0.59268}{-0.801}
\meshline{black}{-0.5126}{0.85411}{-0.555}{0.83146}
\meshline{black}{-0.66845}{-0.73882}{-0.63018}{-0.77023}
\meshline{black}{-0.7071}{-0.7071}{-0.66845}{-0.73882}
\meshline{black}{-0.555}{0.83146}{-0.5937}{0.7998}
\meshline{black}{-0.73756}{-0.66999}{-0.7071}{-0.7071}
\meshline{black}{-0.76833}{-0.63249}{-0.73756}{-0.66999}
\meshline{black}{-0.5937}{0.7998}{-0.63205}{0.76843}
\meshline{black}{-0.79974}{-0.59422}{-0.76833}{-0.63249}
\meshline{black}{-0.83146}{-0.55557}{-0.79974}{-0.59422}
\meshline{black}{-0.63205}{0.76843}{-0.6697}{0.73762}
\meshline{black}{-0.8541}{-0.51322}{-0.83146}{-0.55557}
\meshline{black}{-0.6697}{0.73762}{-0.707}{0.70711}
\meshline{black}{-0.87696}{-0.47044}{-0.8541}{-0.51322}
\meshline{black}{-0.9003}{-0.42678}{-0.87696}{-0.47044}
\meshline{black}{-0.707}{0.70711}{-0.73873}{0.66846}
\meshline{black}{-0.92387}{-0.38268}{-0.9003}{-0.42678}
\meshline{black}{-0.93781}{-0.33673}{-0.92387}{-0.38268}
\meshline{black}{-0.73873}{0.66846}{-0.77014}{0.6302}
\meshline{black}{-0.95189}{-0.29031}{-0.93781}{-0.33673}
\meshline{black}{-0.77014}{0.6302}{-0.80093}{0.59269}
\meshline{black}{-0.80093}{0.59269}{-0.8314}{0.55557}
\meshline{black}{-0.96626}{-0.24294}{-0.95189}{-0.29031}
\meshline{black}{-0.8314}{0.55557}{-0.85498}{0.51148}
\meshline{black}{-0.98078}{-0.19509}{-0.96626}{-0.24294}
\meshline{black}{-0.98549}{-0.1473}{-0.98078}{-0.19509}
\meshline{black}{-0.85498}{0.51148}{-0.87833}{0.46782}
\meshline{black}{-0.99024}{-0.09902}{-0.98549}{-0.1473}
\meshline{black}{-0.87833}{0.46782}{-0.90122}{0.42504}
\meshline{black}{-0.9951}{-0.04976}{-0.99024}{-0.09902}
\meshline{black}{-0.90122}{0.42504}{-0.92387}{0.38268}
\meshline{black}{-0.92387}{0.38268}{-0.93839}{0.33484}
\meshline{black}{-0.93839}{0.33484}{-0.95276}{0.28746}
\meshline{black}{-1}{0}{-0.9951}{-0.04976}
\meshline{black}{-0.95276}{0.28746}{-0.96684}{0.24104}
\meshline{black}{-0.96684}{0.24104}{-0.98078}{0.19509}
\meshline{black}{-0.98078}{0.19509}{-0.98568}{0.14533}
\meshline{black}{-0.99054}{0.09607}{-0.99529}{0.04779}
\meshline{black}{-0.98568}{0.14533}{-0.99054}{0.09607}
\meshline{black}{-0.99529}{0.04779}{-1}{0}
\meshline{red}{1}{0}{0.99529}{-0.04779}
\meshline{red}{1}{0}{0.9951}{0.04976}
\meshline{red}{0.99054}{-0.09606}{0.99529}{-0.04779}
\meshline{red}{0.9951}{0.04976}{0.99025}{0.09903}
\meshline{red}{0.98569}{-0.14533}{0.99054}{-0.09606}
\meshline{red}{0.99025}{0.09903}{0.98549}{0.1473}
\meshline{red}{0.98078}{-0.19509}{0.98569}{-0.14533}
\meshline{red}{0.98549}{0.1473}{0.98078}{0.19509}
\meshline{red}{0.96685}{-0.24104}{0.98078}{-0.19509}
\meshline{red}{0.98078}{0.19509}{0.96627}{0.24294}
\meshline{red}{0.95276}{-0.28746}{0.96685}{-0.24104}
\meshline{red}{0.96627}{0.24294}{0.9519}{0.29031}
\meshline{red}{0.93839}{-0.33483}{0.95276}{-0.28746}
\meshline{red}{0.9519}{0.29031}{0.93781}{0.33673}
\meshline{red}{0.92388}{-0.38268}{0.93839}{-0.33483}
\meshline{red}{0.93781}{0.33673}{0.92387}{0.38268}
\meshline{red}{0.90124}{-0.42503}{0.92388}{-0.38268}
\meshline{red}{0.92387}{0.38268}{0.9003}{0.42678}
\meshline{red}{0.87837}{-0.46781}{0.90124}{-0.42503}
\meshline{red}{0.9003}{0.42678}{0.87696}{0.47044}
\meshline{red}{0.85504}{-0.51147}{0.87837}{-0.46781}
\meshline{red}{0.87696}{0.47044}{0.8541}{0.51322}
\meshline{red}{0.83147}{-0.55557}{0.85504}{-0.51147}
\meshline{red}{0.8541}{0.51322}{0.83146}{0.55557}
\meshline{red}{0.80101}{-0.59269}{0.83147}{-0.55557}
\meshline{red}{0.83146}{0.55557}{0.79974}{0.59422}
\meshline{red}{0.77023}{-0.63018}{0.80101}{-0.59269}
\meshline{red}{0.79974}{0.59422}{0.76833}{0.63249}
\meshline{red}{0.73883}{-0.66845}{0.77023}{-0.63018}
\meshline{red}{0.76833}{0.63249}{0.73756}{0.66999}
\meshline{red}{0.70711}{-0.7071}{0.73883}{-0.66845}
\meshline{red}{0.73756}{0.66999}{0.7071}{0.7071}
\meshline{red}{0.66999}{-0.73756}{0.70711}{-0.7071}
\meshline{red}{0.7071}{0.7071}{0.66839}{0.73875}
\meshline{red}{0.63249}{-0.76834}{0.66999}{-0.73756}
\meshline{red}{0.66839}{0.73875}{0.6301}{0.77006}
\meshline{red}{0.59422}{-0.79974}{0.63249}{-0.76834}
\meshline{red}{0.6301}{0.77006}{0.59263}{0.8007}
\meshline{red}{0.55557}{-0.83146}{0.59422}{-0.79974}
\meshline{red}{0.59263}{0.8007}{0.55557}{0.831}
\meshline{red}{0.51323}{-0.85407}{0.55557}{-0.83146}
\meshline{red}{0.55557}{0.831}{0.51152}{0.85465}
\meshline{red}{0.47045}{-0.87692}{0.51323}{-0.85407}
\meshline{red}{0.51152}{0.85465}{0.46788}{0.87807}
\meshline{red}{0.42679}{-0.90024}{0.47045}{-0.87692}
\meshline{red}{0.46788}{0.87807}{0.42507}{0.90105}
\meshline{red}{0.38268}{-0.9238}{0.42679}{-0.90024}
\meshline{red}{0.42507}{0.90105}{0.38268}{0.9238}
\meshline{red}{0.33673}{-0.93776}{0.38268}{-0.9238}
\meshline{red}{0.38268}{0.9238}{0.33484}{0.93831}
\meshline{red}{0.2903}{-0.95186}{0.33673}{-0.93776}
\meshline{red}{0.33484}{0.93831}{0.28746}{0.95268}
\meshline{red}{0.24293}{-0.96625}{0.2903}{-0.95186}
\meshline{red}{0.28746}{0.95268}{0.24104}{0.96676}
\meshline{red}{0.19509}{-0.98078}{0.24293}{-0.96625}
\meshline{red}{0.24104}{0.96676}{0.19509}{0.9807}
\meshline{red}{0.1473}{-0.98549}{0.19509}{-0.98078}
\meshline{red}{0.19509}{0.9807}{0.14533}{0.98562}
\meshline{red}{0.09902}{-0.99024}{0.1473}{-0.98549}
\meshline{red}{0.14533}{0.98562}{0.09607}{0.9905}
\meshline{red}{0.04976}{-0.9951}{0.09902}{-0.99024}
\meshline{red}{0.09607}{0.9905}{0.04779}{0.99527}
\meshline{red}{0}{-1}{0.04976}{-0.9951}
\meshline{red}{0.04779}{0.99527}{0}{1}
\meshline{red}{-0.05951}{-0.98078}{0}{-1}
\meshline{red}{0}{1}{-0.04976}{0.9951}
\meshline{red}{-0.1026}{-0.97319}{-0.05951}{-0.98078}
\meshline{red}{-0.04976}{0.9951}{-0.09901}{0.99024}
\meshline{red}{-0.14672}{-0.96542}{-0.1026}{-0.97319}
\meshline{red}{-0.09901}{0.99024}{-0.14726}{0.98549}
\meshline{red}{-0.14726}{0.98549}{-0.195}{0.98078}
\meshline{red}{-0.19186}{-0.95747}{-0.14672}{-0.96542}
\meshline{red}{-0.195}{0.98078}{-0.24283}{0.96622}
\meshline{red}{-0.24283}{0.96622}{-0.29013}{0.95183}
\meshline{red}{-0.23803}{-0.94934}{-0.19186}{-0.95747}
\meshline{red}{-0.29013}{0.95183}{-0.33633}{0.93777}
\meshline{red}{-0.28522}{-0.94103}{-0.23803}{-0.94934}
\meshline{red}{-0.33633}{0.93777}{-0.382}{0.92387}
\meshline{red}{-0.33344}{-0.93254}{-0.28522}{-0.94103}
\meshline{red}{-0.382}{0.92387}{-0.4261}{0.90031}
\meshline{red}{-0.38268}{-0.92387}{-0.33344}{-0.93254}
\meshline{red}{-0.42503}{-0.90123}{-0.38268}{-0.92387}
\meshline{red}{-0.4261}{0.90031}{-0.46978}{0.87698}
\meshline{red}{-0.46781}{-0.87837}{-0.42503}{-0.90123}
\meshline{red}{-0.51147}{-0.85503}{-0.46781}{-0.87837}
\meshline{red}{-0.46978}{0.87698}{-0.5126}{0.85411}
\meshline{red}{-0.55557}{-0.83146}{-0.51147}{-0.85503}
\meshline{red}{-0.59268}{-0.801}{-0.55557}{-0.83146}
\meshline{red}{-0.5126}{0.85411}{-0.555}{0.83146}
\meshline{red}{-0.63018}{-0.77023}{-0.59268}{-0.801}
\meshline{red}{-0.66845}{-0.73882}{-0.63018}{-0.77023}
\meshline{red}{-0.7071}{-0.7071}{-0.66845}{-0.73882}
\meshline{red}{-0.555}{0.83146}{-0.5937}{0.7998}
\meshline{red}{-0.73756}{-0.66999}{-0.7071}{-0.7071}
\meshline{red}{-0.76833}{-0.63249}{-0.73756}{-0.66999}
\meshline{red}{-0.5937}{0.7998}{-0.63205}{0.76843}
\meshline{red}{-0.79974}{-0.59422}{-0.76833}{-0.63249}
\meshline{red}{-0.83146}{-0.55557}{-0.79974}{-0.59422}
\meshline{red}{-0.63205}{0.76843}{-0.6697}{0.73762}
\meshline{red}{-0.8541}{-0.51322}{-0.83146}{-0.55557}
\meshline{red}{-0.6697}{0.73762}{-0.707}{0.70711}
\meshline{red}{-0.87696}{-0.47044}{-0.8541}{-0.51322}
\meshline{red}{-0.9003}{-0.42678}{-0.87696}{-0.47044}
\meshline{red}{-0.707}{0.70711}{-0.73873}{0.66846}
\meshline{red}{-0.92387}{-0.38268}{-0.9003}{-0.42678}
\meshline{red}{-0.73873}{0.66846}{-0.77014}{0.6302}
\meshline{red}{-0.93781}{-0.33673}{-0.92387}{-0.38268}
\meshline{red}{-0.95189}{-0.29031}{-0.93781}{-0.33673}
\meshline{red}{-0.77014}{0.6302}{-0.80093}{0.59269}
\meshline{red}{-0.80093}{0.59269}{-0.8314}{0.55557}
\meshline{red}{-0.96626}{-0.24294}{-0.95189}{-0.29031}
\meshline{red}{-0.8314}{0.55557}{-0.85498}{0.51148}
\meshline{red}{-0.98078}{-0.19509}{-0.96626}{-0.24294}
\meshline{red}{-0.98549}{-0.1473}{-0.98078}{-0.19509}
\meshline{red}{-0.85498}{0.51148}{-0.87833}{0.46782}
\meshline{red}{-0.99024}{-0.09902}{-0.98549}{-0.1473}
\meshline{red}{-0.87833}{0.46782}{-0.90122}{0.42504}
\meshline{red}{-0.9951}{-0.04976}{-0.99024}{-0.09902}
\meshline{red}{-0.90122}{0.42504}{-0.92387}{0.38268}
\meshline{red}{-0.92387}{0.38268}{-0.93839}{0.33484}
\meshline{red}{-0.93839}{0.33484}{-0.95276}{0.28746}
\meshline{red}{-0.95276}{0.28746}{-0.96684}{0.24104}
\meshline{red}{-1}{0}{-0.9951}{-0.04976}
\meshline{red}{-0.96684}{0.24104}{-0.98078}{0.19509}
\meshline{red}{-0.98078}{0.19509}{-0.98568}{0.14533}
\meshline{red}{-0.98568}{0.14533}{-0.99054}{0.09607}
\meshline{red}{-0.99529}{0.04779}{-1}{0}
\meshline{red}{-0.99054}{0.09607}{-0.99529}{0.04779}

